Advancing LLM Reasoning Generalists with Preference Trees

We introduce Eurus, a suite of large language models (LLMs) optimized for reasoning. Finetuned from Mistral-7B and CodeLlama-70B, Eurus models achieve state-of-the-art results among open-source models on a diverse set of benchmarks covering mathematics, code generation, and logical reasoning problems. Notably, Eurus-70B beats GPT-3.5 Turbo in reasoning through a comprehensive benchmarking across 12 tests covering five tasks, and achieves a 33.3% pass@1 accuracy on LeetCode and 32.6% on TheoremQA, two challenging benchmarks, substantially outperforming existing open-source models by margins more than 13.3%. The strong performance of Eurus can be primarily attributed to UltraInteract, our newly-curated large-scale, high-quality alignment dataset specifically designed for complex reasoning tasks. UltraInteract can be used in both supervised fine-tuning and preference learning. For each instruction, it includes a preference tree consisting of (1) reasoning chains with diverse planning strategies in a unified format, (2) multi-turn interaction trajectories with the environment and the critique, and (3) pairwise data to facilitate preference learning. UltraInteract allows us to conduct an in-depth exploration of preference learning for reasoning tasks. Our investigation reveals that some well-established preference learning algorithms may be less suitable for reasoning tasks compared to their effectiveness in general conversations. Inspired by this, we derive a novel reward modeling objective which, together with UltraInteract, leads to a strong reward model.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tabs/sft.tex <==
\begin{table}[tbh]
% \vspace{-10pt}
\caption{Overall performance. All test sets except MATH are out-of-distribution to our models and probably most baselines are based on public information, except MAmmoTH, OpenChat, and Starling-LM which have been trained on TheoremQA test sets. \hao{i thought mammoth directly trains on gsm/math?}\lifan{most use gsm, including ours. but gsm plus is a new synthetic dataset released last month} We report pass@1 for coding, accuracy for math, 3-shot accuracy for BBH, and prompt-level loose metric for IFEval. We \sout{strikethrough} the contaminated TheoremQA numbers and average scores. }
% Our UltraLM-Mistral-7B surpasses the 5-times-larger baseline DeepSeek-Coder-34B and our UltraLM-CL-70B is superior to GPT-3.5 Turbo. 
%We report the results of GPT-4 Turbo on coding datasets since we did not find results for GPT-4 Turbo. Our UltraLM-Mistral-7B surpasses Mixtral-MoE and our UltraLM-CL-70B surpasses GPT-3.5 Turbo.}
\label{tab:sft}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}lccccccccccc@{}}
\toprule
\multicolumn{1}{l|}{\multirow{2}{*}{\bf Model}}          & \multicolumn{3}{c|}{\bf Coding}                                                 & \multicolumn{5}{c|}{\bf Math}                                                                                              & \multicolumn{1}{c|}{\bf Reasoning} & \multicolumn{1}{c|}{\bf Ins-Following} & \multicolumn{1}{l}{\multirow{2}{*}{\bf Avg.}} \\ \cmidrule(lr){2-11}
\multicolumn{1}{l|}{}                                & HumanEval            & MBPP                 & \multicolumn{1}{c|}{Leet} & GSM-Plus                & MATH                 & TheoremQA            & SVAMP                & \multicolumn{1}{c|}{ASDiv} & \multicolumn{1}{c|}{BBH} & \multicolumn{1}{c|}{IFEval}        & \multicolumn{1}{l}{}                      


\\ \midrule
\multicolumn{12}{c}{$\sim$7B}                                                                                                                                                                                                                                                                                                                                                       \\ \midrule
\multicolumn{1}{l|}{\textbf{Mistral-Instruct-v0.2}}  & 39.0                 & 30.8                 & \multicolumn{1}{c|}{6.1}      & 15.7                 & 9.5                  & 8.5                  & 42.9                 & \multicolumn{1}{c|}{49.5}  & \multicolumn{1}{c|}{62.4}      & \multicolumn{1}{c|}{44.4}          & 30.9                                      \\
\multicolumn{1}{l|}{\textbf{Zephyr}}                 & 29.3                 & 35.8                 & \multicolumn{1}{c|}{2.2}      & 23.3                 & 5.0                  & 7.8                  & 19.1                 & \multicolumn{1}{c|}{28.0}  & \multicolumn{1}{c|}{61.8}      & \multicolumn{1}{c|}{39.7}          & 25.2                                      \\
\multicolumn{1}{l|}{\textbf{OpenChat-3.5-1210}}      & 64.0                 & 61.7                 & \multicolumn{1}{c|}{11.7}     & 46.7                 & 28.1                 & \sout{19.1}                 & 75.4                 & \multicolumn{1}{c|}{77.0}  & \multicolumn{1}{c|}{67.0}      & \multicolumn{1}{c|}{\textbf{50.3}}          & \sout{50.1}                                      \\
\multicolumn{1}{l|}{\textbf{Starling-LM}}            & 46.3                 & 51.1                 & \multicolumn{1}{c|}{8.9}      & 23.7                 & 21.5                 & \sout{12.0}                 & 26.3                 & \multicolumn{1}{c|}{39.8}  & \multicolumn{1}{c|}{67.1}      & \multicolumn{1}{c|}{26.1}          & \sout{32.3}                                      \\
\multicolumn{1}{l|}{\textbf{MagiCoder-S-DS}}         & 75.6                 & \textbf{70.4}                 & \multicolumn{1}{c|}{\textbf{23.9}}     & 16.4                & 19.9                 & 13.1                & 61.6                 & \multicolumn{1}{c|}{62.8}  & \multicolumn{1}{c|}{57.0}      & \multicolumn{1}{c|}{21.1}          & 42.2                                      \\
\multicolumn{1}{l|}{\textbf{OpenCI-DS-6.7B}}         &   \textbf{76.8}                 &    66.2                  & \multicolumn{1}{c|}{16.1 }         &          41.5            &        31.6              &       16.1               &      74.5                & \multicolumn{1}{c|}{79.8}      & \multicolumn{1}{c|}{53.9}          & \multicolumn{1}{c|}{22.6}              &    47.9                                       \\
\multicolumn{1}{l|}{\textbf{MAmmoTH-Mistral}}        & 24.4                 & 42.4                 & \multicolumn{1}{c|}{7.2}      & 40.1                 & 36.0                 & \sout{26.3}                 & 60.7                 & \multicolumn{1}{c|}{72.3}  & \multicolumn{1}{c|}{57.7}      & \multicolumn{1}{c|}{34.9}          & \sout{40.2}                                      \\
\multicolumn{1}{l|}{\textbf{WizardMath-v1.1}}        & 50.0                 & 53.9                 & \multicolumn{1}{c|}{6.7}      & 54.6                 & 30.0                 & 16.5                 & 57.8                 & \multicolumn{1}{c|}{73.5}  & \multicolumn{1}{c|}{64.4}      & \multicolumn{1}{c|}{22.6}          & 43.0                                     \\
\multicolumn{1}{l|}{\textbf{OpenMath-Mistral}}       & 33.5                 & 46.6                 & \multicolumn{1}{c|}{11.7}     & \textbf{59.4}                 & \textbf{39.1}                 & 13.1                 & 83.4                 & \multicolumn{1}{c|}{79.8}  & \multicolumn{1}{c|}{58.6}      & \multicolumn{1}{c|}{15.0}          & 44.0                                      \\
\rowcolor[HTML]{DAE8FC} 
\multicolumn{1}{l|}{\textbf{Eurus-7B-SFT}}       & 55.5                 & 59.1                 & \multicolumn{1}{c|}{20.0}     & 52.1                & 32.6                 & 20.0                 & 82.2                 & \multicolumn{1}{c|}{84.1}  & \multicolumn{1}{c|}{64.6}      & \multicolumn{1}{c|}{44.0}          & 51.4                                     \\
\rowcolor[HTML]{DAE8FC} 
\multicolumn{1}{l|}{\quad\textbf{+ DPO}}                  & 50.6                 & 52.1                 & \multicolumn{1}{c|}{8.3}      & 51.0                 & 28.3                 & \textbf{20.9}                 & 78.7                 & \multicolumn{1}{c|}{83.8}  & \multicolumn{1}{c|}{65.0}      & \multicolumn{1}{c|}{42.5}          & 48.1                                      \\
\rowcolor[HTML]{DAE8FC} 
\multicolumn{1}{l|}{\quad\textbf{+ KTO}}                  & 56.1                 & 58.6                 & \multicolumn{1}{c|}{18.9}     & 55.0                 & 33.2                 & 20.6                 & 84.4                 & \multicolumn{1}{c|}{85.0}  & \multicolumn{1}{c|}{\textbf{67.6}}      & \multicolumn{1}{c|}{43.1}          & \textbf{52.2}                                      \\
\rowcolor[HTML]{DAE8FC} 
\multicolumn{1}{l|}{\quad\textbf{+ NCA}}                  & 55.5                 & 60.2                 & \multicolumn{1}{c|}{14.4}     & 54.9                 & 34.2                 & \textbf{20.9}                 & \textbf{84.6}                 & \multicolumn{1}{c|}{\textbf{85.4}}  & \multicolumn{1}{c|}{64.3}      & \multicolumn{1}{c|}{42.7}          & 51.7                                      \\ \midrule
\multicolumn{12}{c}{$\sim$40B}                                                                                                                                                                                                                                                                                                                                                      \\ \midrule
\multicolumn{1}{l|}{\textbf{Mixtral-8x7B-Instruct}}  & 50.6                 & 50.1                 & \multicolumn{1}{c|}{5.6}      & \textbf{49.6}                 & \textbf{25.9}                & 20.4                 & 66.4                 & \multicolumn{1}{c|}{68.8}  & \multicolumn{1}{c|}{\textbf{73.5}}      & \multicolumn{1}{c|}{\textbf{48.8}}          & 46.0                                     \\
\multicolumn{1}{l|}{\textbf{DeepSeek-Coder-34B}}     & \textbf{82.3}                & \textbf{73.9}                 & \multicolumn{1}{c|}{\textbf{27.8}}     & 29.5                 & 20.2                 & \textbf{21.9}                 & \textbf{75.2}                 & \multicolumn{1}{c|}{\textbf{85.0}}  & \multicolumn{1}{c|}{61.5}      & \multicolumn{1}{c|}{26.1}          & \textbf{50.3}                                   \\ \midrule
\multicolumn{12}{c}{$\sim$70B}                                                                                                                                                                                                                                                                                                                                                      \\ \midrule
\multicolumn{1}{l|}{\textbf{CodeLLaMA-70B-Instruct}} & 56.7                 & 58.6                 & \multicolumn{1}{c|}{14.4}     & 34.9                 & 12.0                 & 8.4                  & 63.5                 & \multicolumn{1}{c|}{70.1}  & \multicolumn{1}{c|}{74.5}      & \multicolumn{1}{c|}{24.0}          & 41.7                                      \\
\multicolumn{1}{l|}{\textbf{DeepSeek-LM-67B-Chat}}   & 70.7                 & 65.7                 & \multicolumn{1}{c|}{20.0}     & 65.0                 & 41.0                 & 17.9                 & 74.0                 & \multicolumn{1}{c|}{84.0}  & \multicolumn{1}{c|}{78.9}      & \multicolumn{1}{c|}{52.7}          & 57.0                                      \\
\multicolumn{1}{l|}{\textbf{QWen-1.5-72B}}           & 71.3                 & 56.9                 & \multicolumn{1}{c|}{15.6}     & \textbf{65.4}                 & 43.4                 & 18.5                 & 79.5                 & \multicolumn{1}{c|}{79.1}  & \multicolumn{1}{c|}{78.0}      & \multicolumn{1}{c|}{\textbf{53.4}}          & 56.1                                      \\
\multicolumn{1}{l|}{\textbf{OpenCI-CL-70B}}          & 77.4                 & 71.7                & \multicolumn{1}{c|}{20.0}     & 46.1                & 29.2                 & 18.8                 & 76.1                 & \multicolumn{1}{c|}{79.4}  & \multicolumn{1}{c|}{66.7}      & \multicolumn{1}{c|}{26.8}          & 51.2                                      \\
\multicolumn{1}{l|}{\textbf{OpenMath-70B}}           & 39.0                 & 52.6                 & \multicolumn{1}{c|}{15.0}     & 62.2                 & \textbf{45.9}                     & 15.9                 &  86.6                    & \multicolumn{1}{c|}{82.8}      & \multicolumn{1}{c|}{59.9}      & \multicolumn{1}{c|}{15.7}          & 47.6                                      \\
\rowcolor[HTML]{DAE8FC} 
\multicolumn{1}{l|}{\textbf{Eurus-70B-SFT}}    & 75.6                 & \textbf{74.2}                 & \multicolumn{1}{c|}{\textbf{33.3}}     & 58.1                 & 40.6                 & 28.0                 & 86.3                 & \multicolumn{1}{c|}{88.5}  & \multicolumn{1}{c|}{79.9}      & \multicolumn{1}{c|}{49.2}          & 61.4                                      \\
\rowcolor[HTML]{DAE8FC} 
\multicolumn{1}{l|}{\quad\textbf{+ KTO}}                  & 76.8                 & 68.2                 & \multicolumn{1}{c|}{26.1}     & 62.2                & 41.3                 & 30.6                 & \textbf{90.4}                 & \multicolumn{1}{c|}{89.0}  & \multicolumn{1}{c|}{\textbf{80.8}}      & \multicolumn{1}{c|}{46.4}          & 61.2                        \\
\rowcolor[HTML]{DAE8FC} 
\multicolumn{1}{l|}{\quad\textbf{+ NCA}}                  & \textbf{79.3}                 & 71.9                 & \multicolumn{1}{c|}{\textbf{33.3}}     & 62.8                 & 41.7                 & \textbf{32.6}                 & 89.5                 & \multicolumn{1}{c|}{\textbf{90.3}}  & \multicolumn{1}{c|}{80.0}      & \multicolumn{1}{c|}{49.2}          & \textbf{63.1}                                  
 \\ \midrule
\multicolumn{12}{c}{Proprietary Models}                                                                                                                                                                                                                                                                                                                                                      \\ \midrule
\multicolumn{1}{l|}{\textbf{GPT-3.5 Turbo}}  & 76.8                 & 82.5                 & \multicolumn{1}{c|}{23.3}      & 61.2                 & 37.8                 & 35.6                 & 83.0                 & \multicolumn{1}{c|}{90.6}  & \multicolumn{1}{c|}{70.1}      & \multicolumn{1}{c|}{56.6}          & 61.8                                     \\
\multicolumn{1}{l|}{\textbf{GPT-4}}     & \textbf{85.4}                & \textbf{83.5}                 & \multicolumn{1}{c|}{\textbf{41.8}}     & \textbf{85.6}                 & \textbf{69.7}                 & \textbf{52.4}                 & \textbf{94.8}                 & \multicolumn{1}{c|}{\textbf{92.6}}  & \multicolumn{1}{c|}{\textbf{86.7}}      & \multicolumn{1}{c|}{\textbf{79.7}}          & \textbf{76.2}

\\ \bottomrule
\end{tabular}
}
\vspace{-10pt}
\end{table}

==> tabs/stats.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[tbh]
\caption{Some statistics of \dataname. \hanbin{need to update. as well as the table in appendix}}
\resizebox{\textwidth}{!}{

\begin{tabular}{@{} lccccccccccc @{}}
\toprule
\multirow{2}{*}{\textbf{Task}}   & \multicolumn{2}{c}{\textbf{Type}}                         & \multirow{2}{*}{\textbf{\# Instructions}} & \multicolumn{5}{c}{\textbf{\# Turns per Traj.}}                     & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Avg.\\  \# Turns\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\# Tokens \\ per Traj.\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Total \\ \# Pairs\end{tabular}}} \\ \cline{2-3} \cline{5-9}
                                 & \textbf{w/ Interaction?}    & \textbf{w/ Tool?}           &                                           & \textbf{T1} & \textbf{T2} & \textbf{T3} & \textbf{T4} & \textbf{T5} &                                                                                    &                                                                                          &                                                                                     \\ \midrule
\multirow{4}{*}{\textbf{Math}}   & \Checkmark   & \Checkmark   & 22,928                                    & 10,440      & 4,122       & 1,898       & 904         & 5,564       & 2.4                                                                                & 1,750.0                                                                                  & 42,780                                                                              \\
                                 & \XSolidBrush   & \Checkmark & 2,757                                     & 2,757       & -           & -           & -           & -           & 1.0                                                                                & 509.0                                                                                    & 13,217                                                                              \\
                                 & \Checkmark & \XSolidBrush   & 22,639                                    & 10,708      & 3,521       & 1,459       & 723         & 6,228       & 2.5                                                                                & 1,521.9                                                                                  & 44,750                                                                              \\
                                 & \XSolidBrush & \XSolidBrush & 2,083                                     & 2,083       & -           & -           & -           & -           & 1.0                                                                                & 574.7                                                                                    & 12,624                                                                              \\ \midrule
\multirow{2}{*}{\textbf{Coding}} & \Checkmark   & -                           & 20,463                                    & 13,265      & 2,584       & 987         & 379         & 3,248       & 1.9                                                                                & 1,728.5                                                                                  & 18,106                                                                              \\
                                 & \XSolidBrush & -                           & 8,495                                     & 8,495       & -           & -           & -           & -           & 1.0                                                                                & 1,228.4                                                                                  & 78,636                                                                              \\ \midrule
\multirow{2}{*}{\textbf{Logic}}           & \Checkmark   & \Checkmark   & 2,086                                     & 1,685       & 298         & 72          & 8           & 23          & 1.3                                                                                & 1,299.8                                                                                  & 1,750                                                                               \\
                                 & \Checkmark   & \XSolidBrush & 4,467                                     & 2,453       & 1,674       & 340         & 0           & 0           & 1.5                                                                                & 1,266.7                                                                                  & 7,958                                                                               \\ \midrule
\textbf{Total}                   & -                           & -                           & 85,918                                    & 51,886      & 12,199      & 4,756       & 2,014       & 15,063      & 1.6                                                                                & 1,227.1                                                                                  & 219,821                                                                             \\ \bottomrule
\end{tabular}
}
\label{tab:stats}

\end{table*}

==> tabs/stats_dataset_breakdown.tex <==
\begin{table}[]
\caption{Stats breakdown \lifan{code alpaca->MagiCoder}}
\label{tab:stats_breakdown}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}l|cccccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Task}} & \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{w/ Tool?}} & \multirow{2}{*}{\textbf{\# Instructions}} & \multirow{2}{*}{\textbf{\# Pairs}} & \multirow{2}{*}{\textbf{Avg. \# Turn}} & \multirow{2}{*}{\textbf{Avg. Length}} & \multicolumn{2}{c}{\textbf{Human Annotation}}           \\ \cmidrule(l){8-9} 
                               &                                   &                                    &                                           &                                    &                                        &                                       & \textbf{Has Answer?}      & \textbf{Has Rationale?}     \\ \midrule
\multirow{9}{*}{Math}          & \multirow{2}{*}{GSM8K}            & \Checkmark          & 4,522                                     & 10,277                             & 2.4                                    & 1,746.7                               & \Checkmark & \Checkmark   \\
                               &                                   & \XSolidBrush        & 7,257                                     & 10,879                             & 1.6                                    & 823.3                                 & \Checkmark & \Checkmark   \\
                               & \multirow{2}{*}{MATH}             & \Checkmark          & 7,474                                     & 22,905                             & 1.8                                    & 1,189.0                               & \Checkmark & \Checkmark   \\
                               &                                   & \XSolidBrush        & 7,471                                     & 25,765                             & 2.4                                    & 1,735.0                               & \Checkmark & \Checkmark   \\
                               & \multirow{2}{*}{MathQA}           & \Checkmark          & 7,552                                     & 15,079                             & 3.1                                    & 2,338.5                               & \Checkmark & \Checkmark   \\
                               &                                   & \XSolidBrush        & 7,159                                     & 17,743                             & 3.2                                    & 1,916.3                               & \Checkmark & \Checkmark   \\
                               & \multirow{2}{*}{NumGlue}          & \Checkmark          & 3,020                                     & 3,601                              & 2.4                                    & 1,474.6                               & \Checkmark & \XSolidBrush \\
                               &                                   & \XSolidBrush        & 2,835                                     & 2,987                              & 2.1                                    & 1,056.1                               & \Checkmark & \XSolidBrush \\
                               & TabMWP                            & \Checkmark          & 3,117                                     & 4,135                              & 1.4                                    & 842.6                                 & \Checkmark & \XSolidBrush \\ \midrule
\multirow{3}{*}{Logic}         & Reclor                            & \XSolidBrush        & 4,467                                     & 7,958                              & 1.5                                    & 1,266.7                               & \Checkmark & \XSolidBrush \\
                               & HotpotQA                          & \Checkmark          & 1,182                                     & 1,009                              & 1.3                                    & 1,333.2                               & \Checkmark & \XSolidBrush \\
                               & StrategyQA                        & \Checkmark          & 904                                       & 741                                & 1.3                                    & 1,256.2                               & \Checkmark & \XSolidBrush \\ \midrule
\multirow{4}{*}{Coding}        & Alphacode                         & -                                  & 8,167                                     & 44,319                             & 1.8                                    & 2,061.7                               & \Checkmark & \Checkmark   \\
                               & Taco                              & -                                  & 9,016                                     & 50,877                             & 1.9                                    & 2,143.5                               & \Checkmark & \Checkmark   \\
                               & WikiTable                         & -                                  & 1,401                                     & 1,544                              & 2.1                                    & 1,794.8                               & \Checkmark & \XSolidBrush \\
                               & Code Alpaca                       & -                                  & 10,374                                    & 0                                  & 1.2                                    & 687.1                                 & \XSolidBrush & \XSolidBrush \\ \bottomrule

\end{tabular}
}
\end{table}
